Approximation Algorithms for Socially Fair Clustering

We present an $(e^{O(p)} \frac{\log \ell}{\log\log\ell})$-approximation algorithm for socially fair clustering with the $\ell_p$-objective. In this problem, we are given a set of points in a metric space. Each point belongs to one (or several) of $\ell$ groups. The goal is to find a $k$-medians, $k$-means, or, more generally, $\ell_p$-clustering that is simultaneously good for all of the groups. More precisely, we need to find a set of $k$ centers $C$ so as to minimize the maximum over all groups $j$ of $\sum_{u \text{ in group }j} d(u,C)^p$. The socially fair clustering problem was independently proposed by Ghadiri, Samadi, and Vempala [2021] and Abbasi, Bhaskara, and Venkatasubramanian [2021]. Our algorithm improves and generalizes their $O(\ell)$-approximation algorithms for the problem. The natural LP relaxation for the problem has an integrality gap of $\Omega(\ell)$. In order to obtain our result, we introduce a strengthened LP relaxation and show that it has an integrality gap of $\Theta(\frac{\log \ell}{\log\log\ell})$ for a fixed $p$. Additionally, we present a bicriteria approximation algorithm, which generalizes the bicriteria approximation of Abbasi et al. [2021].

==> hardness.tex <==
\section{Hardness of Approximation for Generalized $\ell_{p,q}$-Clustering}\label{sec:hardness}
In this section we show that the $\ell_{p,\infty}$-clustering problem is $\Omega(\log \ell)$-hard to approximate unless ${\bf P} = \NP$ where $\ell$ is the number of groups. First, we prove that a variant of the {\em set cover} problem denoted as {\em min-max coverage set cover} is $\Omega(\log n)$-hard where $n$ is the number of items in the set system. Then, we show a reduction from the min-max coverage set cover problem to the $\ell_{p,\infty}$-clustering problem.

\begin{definition}[Minimum Multicover]\label{def:min-multicover}
Given a collection of $m$ sets $\sF = \{S_1, \cdots, S_m\}$ each a subset of a ground set $\sU = \{e_1, \cdots, e_n\}$ and a budget constraint $t$, the goal is find $\sC \subseteq \sF$ of size $t$ such that maximum number of times that an item of $\sU$ is covered by $\sC$ is minimized.  
\end{definition} 

\begin{theorem}\label{thm:hard-min-max-sc}
Given a set system $(\sF, \sU)$ where $|\sF| = m$ and $|\sU| = n$, the minimum multicover problem is $\Omega(\log n)$-hard to approximate unless ${\bf P} = \NP$.
\end{theorem}
\begin{proof}
%The proof exploits an instance similar to the standard hardness instance of the set cover problem by Lund and Yannakakis~\cite{lund1994hardness} and Feige~\cite{feige1998threshold}. Roughly speaking, in the instance reduced to {\em label cover} instance to show the hardness of set cover, in one case there exists $k$ disjoint sets $S_1, \cdots, S_k$ each of size $n/k$ that covers $\sU$ while in the other case at least $\Omega(k\log n)$ sets of size $n/k$ are need to cover $\sU$. Hence, the same instance shows the $\Omega(\log n)$-hardness of min-max coverage set cover.
%
%Using the recent result of Dinur and Steurer~\cite{dinur2014analytical}, the described hardness of approximation is under ${\bf P} \neq \NP$.  
\end{proof}

Next, we show an approximation preserving reduction from the min-max coverage set cover problem to the $\ell_{p,\infty}$-clustering problem.

\begin{theorem}\label{thm:hardness-gen-clustering}
It is $\NP$-hard to approximate he $\ell_{p, \infty}$-clustering problem over $\ell$ groups within a factor of $o(\log \ell)$. 
\end{theorem}
\begin{proof}
Given an instance of set cover $S_1, \cdots, S_m \subseteq [\ell]$, we construct an instance $\sI$ of the $\ell_{p,\infty}$-clustering with $\ell$ groups as follows:
\begin{itemize}
\item there is a point $o_i$ corresponding to each set $S_i$ in the input,
\item the point $o_i$ belongs to group $P_j$ if $j\in S_i$,
\item there is a unique root node s.t. for each point $o_i$, $d(o_i, r) = 1$ and for each pair of points $o_i, o_j$, $d(o_i, o_j)=2$.  
\end{itemize}
To summarize, $\sI$ consists of $m+1$ points and $\ell$ groups and the distance function $d$ defines a metric space.

Next, we show that the minimum value of maximum coverage of any item in $[\ell]$ subject to the constraint that we pick $t$ sets from $S_1, \cdots, S_m$ is equal to the optimal cost of $\ell_{p, \infty}$-clustering of the constructed instance.
\end{proof}




==> prefix_cls.tex <==

\numberwithin{figure}{section}
\numberwithin{table}{section}
\numberwithin{equation}{section}%

%----    Handling references - end



\newenvironment{inline}{\begin{center}\footnotesize\sf}{\end{center}}
%\renewcommand{\arraystretch}{1.2}
\theoremstyle{plain}%
\newtheorem{theorem}{Theorem}[section]

\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim} \newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{invariant}[theorem]{Invariant}
\newtheorem{question}[theorem]{Question}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{openproblem}[theorem]{Open Problem}
\newtheorem{definition}[theorem]{Definition}


\theoremstyle{plain}%
\theoremheaderfont{\bf} \theorembodyfont{\upshape}%
\newtheorem{remark}[theorem]{Remark}%
\newtheorem*{remark:unnumbered}[theorem]{Remark}%
\newtheorem*{remarks}[theorem]{Remarks}%
\newtheorem{defn}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{xca}[theorem]{Exercise}
\newtheorem{exercise_h}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}%

% Proof environment

\theoremheaderfont{\em}%
\theorembodyfont{\upshape}%
\theoremstyle{nonumberplain}%
\theoremseparator{}%
\theoremsymbol{\myqedsymbol}%
\newtheorem{proof}{Proof:}%

%\newcommand{\myqedsymbol}{\rule{2mm}{2mm}}
\newcommand{\myqedsymbol}{$\square$}

\newtheorem{proofof}{Proof of\!}%
%\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}

\newcommand{\eps}{\varepsilon}%
\def\bar{\overline}
\def\floor#1{\lfloor {#1} \rfloor}
\def\ceil#1{\lceil {#1} \rceil}
\def\script#1{\mathcal{#1}}
\def\etal{\text{et al.}\xspace}
\def\Union{\bigcup}
\def\sep{\;|\;}
\def\card#1{|#1|}
\def\set#1{\{#1\}}
\def\E{\mathbf{E}}
\def\Var{\mathbf{Var}}

%\def\arc#1{\accentset{\rightharpoonup}{#1}}

\newcommand{\argmax}{\mathrm{argmax}{}\xspace}
\newcommand{\argmin}{\mathrm{argmin}{}\xspace}

\def\wrt{\text{w.r.t.}\xspace}

\newcommand{\polylog}{\mathop{\mathrm{polylog}}}%
\newcommand{\poly}{\mathop{\mathrm{poly}}}%

\def\whp{\text{w.h.p.}}
\newcommand{\tldO}{\widetilde{O}}%
\newcommand{\tldOmega}{\widetilde{\Omega}}%
\newcommand{\tldTheta}{\widetilde{\Theta}}%


\def\sA{\script{A}}
\def\sB{\script{B}}
\def\sC{\script{C}}
\def\sD{\script{D}}
\def\sF{\script{F}}
\def\sG{\script{G}}
\def\sI{\script{I}}
\def\sL{\script{L}}
\def\sK{\script{K}}
\def\sM{\script{M}}
\def\sN{\script{N}}
\def\sO{\script{O}}
\def\sQ{\script{Q}}
\def\sS{\script{S}}
\def\sT{\script{T}}
\def\sU{\script{U}}
\def\sV{\script{V}}
\def\sY{\script{Y}}
\def\sW{\script{W}}
\def\sZ{\script{Z}}

\def\NP{\ensuremath{\mathrm{\mathbf{NP}}}}
%\def\cost{\mathrm{cost}}
\def\dist{\mathrm{dist}}
\def\lp{\script{LP}}
\def\nn{\mathrm{NN}}
\def\cllp{ClusterLP}
\def\optcllp{BasicClusterLP}
\def\spcllp{SparseClusterLP}
\def\opt{\textsc{OPT}}
\def\rem{\mathrm{rem}}


\def\clcp{\textbf{Cluster-CP}}
\def\optclcp{\textbf{Cluster-CP-I}}
\def\optclcpsp{\textbf{Cluster-CP-II}}
\def\spclcp{\textbf{Sparse-Cluster-CP}}


\newcommand\faircost{{\operatorname{fair-cost}}}
\newcommand\cost{{\operatorname{cost}}}
\newcommand\vol{{\operatorname{vol}}}
\def\R{\script{R}}
\newcommand{\sol}{\textsc{SOL}}%
\def\Y{\boldsymbol{Y}}
\def\X{\boldsymbol{X}}
\def\g{{\boldsymbol{g}}}

